A Survey on Industrial Control System Testbeds and Datasets for Security Research

The increasing digitization and interconnection of legacy Industrial Control Systems (ICSs) open new vulnerability surfaces, exposing such systems to malicious attackers. Furthermore, since ICSs are often employed in critical infrastructures (e.g., nuclear plants) and manufacturing companies (e.g., chemical industries), attacks can lead to devastating physical damages. In dealing with this security requirement, the research community focuses on developing new security mechanisms such as Intrusion Detection Systems (IDSs), facilitated by leveraging modern machine learning techniques. However, these algorithms require a testing platform and a considerable amount of data to be trained and tested accurately. To satisfy this prerequisite, Academia, Industry, and Government are increasingly proposing testbed (i.e., scaled-down versions of ICSs or simulations) to test the performances of the IDSs. Furthermore, to enable researchers to cross-validate security systems (e.g., security-by-design concepts or anomaly detectors), several datasets have been collected from testbeds and shared with the community. In this paper, we provide a deep and comprehensive overview of ICSs, presenting the architecture design, the employed devices, and the security protocols implemented. We then collect, compare, and describe testbeds and datasets in the literature, highlighting key challenges and design guidelines to keep in mind in the design phases. Furthermore, we enrich our work by reporting the best performing IDS algorithms tested on every dataset to create a baseline in state of the art for this field. Finally, driven by knowledge accumulated during this survey's development, we report advice and good practices on the development, the choice, and the utilization of testbeds, datasets, and IDSs.

==> backup.tex <==
\renewcommand{\arraystretch}{1.3}
%\begin{landscape}
\begin{center}
\footnotesize
\tablecaption{Summary of testbeds presented in the literature. We denote \textbf{Category} as H: Hybrid, P: Physical, and V: Virtual. To specify the ICS process \textbf{Physics} we use S: Simulated, R: Real, M: Mixed, and No: if there is not a physical process. To denote the \textbf{License}, we use OD: Open Description, E: Education, OS: Open-Source, C: Collaboration, and NA: Not Available. To denote the \textbf{Scope}, we use S: Security, G: General, P: Pedagogy, and F: Forensic. To denote the \textbf{Cost} we use L: Low, M: Medium, and H: High.}
\tablefirsthead{%
\hline
\rowcolor[HTML]{EFEFEF} 
\rotatebox{-25}{\textbf{Name or authors}}                & \rot{\textbf{Category}} & \rot{\textbf{Institution\space}}    & \rot{\textbf{Country}} & \rot{\textbf{Sector}} & \rot{\textbf{Physics}} & \rot{\textbf{License}} & \rot{\textbf{Scope}} & \rot{\textbf{Cost}} & \rot{\textbf{Reference}}            & \rot{\textbf{Resource}}              \\ \hline

}

\tablehead{%
    \multicolumn{11}{c}%
    {{\bfseries \tablename~\thetable{} -- continued from previous page}} \\
    \hline
    \rowcolor[HTML]{EFEFEF} 
    \rotatebox{-25}{\textbf{Name or authors}}                & \rot{\textbf{Category}} & \rot{\textbf{Institution\space}}    & \rot{\textbf{Country}} & \rot{\textbf{Sector}} & \rot{\textbf{Physics}} & \rot{\textbf{License}} & \rot{\textbf{Scope}} & \rot{\textbf{Cost}} & \rot{\textbf{Reference}}            & \rot{\textbf{Resource}}              \\ \hline
}

\tabletail{%
    \hline
}
\begin{supertabular}[l]{|l|l|l|l|l|l|l|l|l|l|l|}
%

\rowcolor[HTML]{FFFFC7} 
\textbf{Aghamolki et al.}    & H                       & USF                     & Florida, US      & Power Grid            & S                      & OD                     & S                    & M                   & \cite{7335093}                 & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{Alves et al.}        & H                       & UAH                     & Alabama, US      & Gas Pipeline          & S                      & OD                     & S                    & L                   & \cite{alves2016virtualization} & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{CockpitCI}           & H                       & University of Coimbra   & Portugal         & Power Grid            & S                      & OD                     & S                    & M                   & \cite{7542169}                 & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{CyberCity}           & H                       & SANS Institute          & -                & City                  & M                      & E                      & S, P                 & H                   & \cite{BorgesHink2016}          & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{EPIC (IPSC)}         & H                       & JRC Ispra               & Italy            & General CPS           & S                      & OS                     & S                    & L                   & \cite{Siaterlis2013epic}       & \cite{EpicWeb}                   \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{EPS-ICS}             & H                       & BIT                     & China            & Generic ICS           & R                      & NA                     & G                    & L                   & \cite{Gao2013eps}              & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{Gillen et al.}       & H                       & ORNL                    & Tennessee, US    & Cooling System        & S                      & OD                     & S                    & M                   & \cite{Gillen2020}              & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{Hui Nuclear}         & H                       & Queen's University      & UK               & Nuclear Plant         & S                      & OD                     & S                    & M                   & \cite{Hui2019hybrid}           & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{HYDRA}               & H                       & University of Roma Tre  & Italy            & Water Distribution    & R                      & OS                     & S                    & L                   & \cite{Bernieri2016hydra}       & \cite{HYDRAWeb}                  \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{Jarmakiewicz et al.} & H                       & MUT                     & Poland           & Power Grid            & S                      & OD                     & G                    & M                   & \cite{7158687}                 & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{Kaouk et al.}        & H                       & University of Grenoble  & France           & Generic ICS           & S                      & OD                     & S                    & L                   & \cite{kaouk2018testbed}        & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{Kim et al.}          & H                       & NSRI                    & South Korea      & 6 Different ICS       & R                      & E                      & S, P                 & H                   & \cite{Kim2019}                 & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{Koutsandria et al.}  & H                       & Sapienza University     & Italy            & Power Grid            & S                      & OD                     & S, F                 & M                   & \cite{koutsandria2015real}     & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{KYPO4INDUSTRY}       & H                       & Masaryk University      & Czech Republic   & Linear Motor          & R                      & OD                     & P                    & M                   & \cite{Celeda2020krypto}        & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{LegoSCADA}           & H                       & Universite Paris-Saclay & France           & Vehicular             & R                      & OS                     & S                    & L                   & \cite{Rubio2017lego}           & \cite{LegoSCADAWeb}              \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{Microgrid}           & H                       & OSU                     & Ohio, US         & Power Grid            & M                      & OD                     & G, P                 & M                   & \cite{Guo2013}                 & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{MSICST}              & H                       & -                       & China            & 4 Different ICS       & S                      & OD                     & S                    & H                   & \cite{xu2019msicst}            & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{NIST}                & H                       & USDOC                   & US               & 4 Different ICS       & M                      & C                      & S                    & M                   & \cite{Testbed2015nist}         & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{PNNL}                & H                       & PNNL                    & Washington, US   & Generic CPS           & S                      & OD                     & S                    & L                   & \cite{Edgar2011}               & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{Queiroz et al.}      & H                       & RMIT University         & Australia        & Water Distribution    & R                      & OD                     & S                    & L                   & \cite{Queiroz2009}             & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{SNL Testbed}         & H                       & SNL                     & New Mexico, US   & Generic ICS           & No                     & OD                     & S                    & L                   & \cite{Urias2012}               & -                                \\ \hline
\rowcolor[HTML]{FFFFC7} 
\textbf{VPST}                & H                       & University of Illinois  & Illinois, US     & Power Grid            & S                      & OD                     & S, G                 & L                   & \cite{Bergman2009}             & -                                \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{Ahmed et al.}        & P                       & UNO                     & Louisiana, US    & 3 Different ICS       & R                      & OD                     & S, F, P              & M                   & \cite{Ahmed2016}               & -                                \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{Blazek et al.}       & P                       & BUT                     & Czech Republic   & Power Grid            & R                      & OD                     & S                    & M                   & \cite{blazek2019development}   & -                                \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{BU-Testbed}          & P                       & Binghamton University   & New York, US     & Power Plant           & R                      & OD                     & S                    & M                   & \cite{korkmaz2016industrial}   & -                                \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{EPIC (iTrust)}       & P                       & SUTD                    & Singapore        & Electric Power        & R                      & E                      & S                    & H                   & \cite{Adepu2018epic}           & \cite{iTrustEPICWeb}             \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{HAI Testbed}         & P                       & ETRI                    & South Korea      & Power Plant           & R                      & OD                     & S                    & H                   & \cite{Shin2019}                & -                                \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{Lancaster's}         & P                       & Lancaster University    & UK               & Generic ICS           & R                      & C                      & G, P                 & H                   & \cite{Green2017pains}          & -                                \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{LICSTER}             & P                       & HS-Augsburg             & Germany          & Generic ICS           & R                      & OS                     & S, P                 & L                   & \cite{sauer2019licster}        & -                                \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{Mississipi Ethernet} & P                       & MSU                     & Mississippi, US  & 2 different ICS       & R                      & E                      & S, P                 & M                   & \cite{Morris2011testbeds}      & -                                \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{Mississipi Serial}   & P                       & MSU                     & Mississippi, US  & Industrial op.s       & R                      & E                      & S, P                 & M                   & \cite{Morris2011testbeds}      & -                                \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{PowerCyber}          & P                       & Iowa State University   & Iowa, US         & Power Grid            & R                      & OD                     & S, P                 & L                   & \cite{Hahn2010}                & -                                \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{Sayegh et al.}       & P                       & AUB                     & Lebanon          & Generic ICS           & No                     & OD                     & S                    & M                   & \cite{sayegh2013internal}      & -                                \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{SGTB}                & P                       & INL                     & Idaho, US        & Power Grid            & R                      & NA                     & S                    & H                   & \cite{INL2017}                 & -                                \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{SWaT}                & P                       & SUTD                    & Singapore        & Water Treatment       & R                      & C                      & S                    & H                   & \cite{Mathur2016swat}          & \cite{iTrustSWATWeb} \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{Teixeira et. al}     & P                       & IFET                    & Brazil           & Water Distribution    & R                      & OD                     & S                    & M                   & \cite{Teixeira2018}            & -                                \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{T-GPP}               & P                       & JRC Ispra               & Italy            & Power Plant           & R                      & OD                     & S                    & H                   & \cite{Fovino2010}              & -                                \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{WADI}                & P                       & SUTD                    & Singapore        & Water Distribution    & R                      & C                      & S, P                 & H                   & \cite{Ahmed2017wadi}           & \cite{iTrustWADIWeb}             \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{Yang et al.}         & P                       & QUB                     & Irland           & Power Grid            & R                      & OD                     & S                    & M                   & \cite{6737311}                 & -                                \\ \hline
\rowcolor[HTML]{ECF4FF} 
\textbf{Zhang et al.}        & P                       & University of Tennessee & Tennessee, US    & Nuclear Plant         & R                      & OD                     & S                    & M                   & \cite{Zhang2019}               & -                                \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{Davis et al.}        & V                       & University of Illinois  & Illinois, US     & Power Grid            & S                      & OD                     & S                    & L                   & \cite{Davis2006}               & -                                \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{DVCP}                & V                       & TUHH                    & Germany          & Chemical Process      & S                      & OS                     & S, F                 & L                   & \cite{krotofil2015rocking}     & \cite{DVCP-TEWeb}   \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{Farooqui et al.}     & V                       & NUST                    & Pakistan         & Generic CPS           & S                      & OD                     & S                    & L                   & \cite{farooqui2014cyber}       & -                                \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{Gas Pipeline}        & V                       & MSU                     & Mississippi, US  & Gas Pipeline          & S                      & NA                     & S                    & L                   & \cite{Morris2015}              & -                                \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{Genge et al.}        & V                       & JRC Ispra               & Italy            & Generic ICS           & S                      & OD                     & S                    & L                   & \cite{Genge2012}               & -                                \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{Giani et al.}        & V                       & UC Berkeley             & -                & Generic ICS           & S                      & OD                     & S                    & L                   & \cite{Giani2008}               & -                                \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{GRFICS}              & V                       & Georgia Tech            & Georgia, US      & Chemical Process      & S                      & OS                     & S, P                 & L                   & \cite{formby2018lowering}      & \cite{GRFICSWeb}                 \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{Jin et al.}          & V                       & UIUC                    & Illinois, US     & Generic ICS           & S                      & OD                     & S                    & L                   & \cite{jin2011event}            & -                                \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{Koganti et al.}      & V                       & University of Idaho     & Idaho, US        & Power Grid            & S                      & OD                     & S                    & L                   & \cite{8323960}                 & -                                \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{Lee et al.}          & V                       & Ajou University         & Korea            & Power Plant           & S                      & OD                     & S                    & L                   & \cite{lee2018design}           & -                                \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{Maynard SCADA}       & V                       & Queen's University      & UK               & Generic ICS           & S                      & OS                     & S                    & L                   & \cite{Maynard2018open}         & \cite{MaynardWeb}                \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{MiniCPS}             & V                       & SUTD                    & Singapore        & Generic CPS           & S                      & OS                     & S                    & L                   & \cite{Antonioli2015mini}       & \cite{MiniWeb}                   \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{Reavers \& Morris}   & V                       & Georgia Tech            & Georgia, US      & Generic ICS           & S                      & OD                     & S                    & L                   & \cite{Reaves2012virtual}       & -                                \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{RICS-el}             & V                       & Chalmers University     & Sweden           & Power Grid            & S                      & OD                     & S                    & L                   & \cite{Almgren2019}             & -                                \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{SCADA-SST}           & V                       & KFUPM                   & Saudi Arabia     & 2 different ICS       & S                      & OS                     & S                    & L                   & \cite{ghaleb2016scada}         & \cite{GhalebWeb}                 \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{SCADASim}            & V                       & RMIT University         & Australia        & Generic ICS           & S                      & OS                     & S                    & L                   & \cite{Queiroz2011}             & \cite{SCADASimWeb}               \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{SCADAVT}             & V                       & RMIT University         & Australia        & Water Distribution    & S                      & OD                     & S                    & L                   & \cite{Almalawi2013}            & -                                \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{Singhet et al.}      & V                       & C-DAC                   & India            & Power Grid            & S                      & OD                     & S                    & L                   & \cite{singh2015testbed}        & -                                \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{TASSCS}              & V                       & University of Arizona   & Arizona, US      & Power Grid            & S                      & OD                     & S                    & L                   & \cite{Mallouhi2011}            & -                                \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{VTET}                & V                       & SKL-MEAC                & China            & Chemical Process      & S                      & OD                     & S                    & L                   & \cite{Xie2018vtet}             & -                                \\ \hline
\rowcolor[HTML]{DFFFE0} 
\textbf{Wang et al.}         & V                       & Tsinghua University     & China            & Generic ICS           & S                      & OD                     & S                    & L                   & \cite{Wang2010}                & -                                \\ \hline

\end{supertabular}
\label{tab:testbed}
\end{center}
